Ultimate TreeAutomizer (CHC-COMP Tool Description)

We present Ultimate TreeAutomizer, a solver for satisfiability of sets of constrained Horn clauses. Constrained Horn clauses (CHC) are a fragment of first order logic with attractive properties in terms of expressiveness and accessibility to algorithmic solving. Ultimate TreeAutomizer is based on the techniques of trace abstraction, tree automata and tree interpolation. This paper serves as a tool description for TreeAutomizer in CHC-COMP 2019.

==> eptcsdata.tex <==
\providecommand{\firstpage}{42}
\providecommand{\publicationstatus}{E. De Angelis, G. Fedyukovich, N. Tzevelekos and M. Ulbrich (Eds.):\\
Sixth Workshop on Horn Clauses for Verification and Synthesis and\\ 
Third Workshop on Program Equivalence and Relational Reasoning.\\
EPTCS 296, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.296.7}{10.4204/EPTCS.296.7}}

